Real-Time Document Image Classification using Deep CNN and Extreme Learning Machines

This paper presents an approach for real-time training and testing for document image classification. In production environments, it is crucial to perform accurate and (time-)efficient training. Existing deep learning approaches for classifying documents do not meet these requirements, as they require much time for training and fine-tuning the deep architectures. Motivated from Computer Vision, we propose a two-stage approach. The first stage trains a deep network that works as feature extractor and in the second stage, Extreme Learning Machines (ELMs) are used for classification. The proposed approach outperforms all previously reported structural and deep learning based methods with a final accuracy of 83.24% on Tobacco-3482 dataset, leading to a relative error reduction of 25% when compared to a previous Convolutional Neural Network (CNN) based approach (DeepDocClassifier). More importantly, the training time of the ELM is only 1.176 seconds and the overall prediction time for 2,482 images is 3.066 seconds. As such, this novel approach makes deep learning-based document classification suitable for large-scale real-time applications.

==> intro_zee.tex <==
\section{Introduction}
%Document classification is traditionally considered an important task in various Document Image Processing Pipelines (DIPP), such as in document retrieval, information extraction, and text recognition.  An initial classification of documents into different known classes not only simplifies various document processing tasks but also increases the overall performance of document processing systems~\cite{doclass_Dengel95}. To date, most of the document classification methods generally use either text content or document structure to categorize documents into different classes,  like contracts, letters, forms, essays, memos, insurance documents, etc. The paper at hand addresses document classification problem by considering the overall structure of document rather than the content.

The document image processing pipeline (DIPP) entails an important step known as document image classification (ref).
It plays an important role in document retrieval (ref), information extraction (ref), and text recognition (ref). 
Dengel et al.~\cite{doclass_Dengel95} in their work signify the importance of this step both that it does not only simplify the following tasks in DIPP and also results in overall improvement.
In order to classify the document into different categoris the paper at hand uses a 2-phase approach.
The first phase is the training of a deep neural network that will be used as feature extractor.
In the second phase Extreme Learning Machines (ELMs) are employed.



% \begin{figure}[!b]
% \captionsetup[subfigure]{labelformat=empty}
%   \subfloat[(a)]{\includegraphics[width=\columnwidth]{OurCases.png}}\\
%  \subfloat[(b)]{\includegraphics[width=\columnwidth]{Fig1c.png}}
% \caption{(a) Sample images from the ImageNet database. (b) Sample images from the Tobacco-3482 Legislation database on whom the proposed system is evaluated.}
% \label{fig:ImageNet}}
% \end{figure}

% \begin{figure*}
% \centering
% \captionsetup[subfigure]{labelformat=empty}
%   \subfloat[(a)]{\includegraphics[width=0.31\textwidth]{Adv.png}}
% 	\hspace{0.2cm}
%  \subfloat[(b)]{\includegraphics[width=0.31\textwidth]{Form.png}}
%  \hspace{0.2cm}
%  \subfloat[(c)]{\includegraphics[width=0.31\textwidth]{Scientific.png}}
% \caption{Example document images from the Tobacco-3482 Legislation dataset highlighting intra-class variations. Three classes are depicted for reference: (a) Ads, (b) Forms, and (c) Scientific writings.}
% \label{fig:TobaccoDoc}}
% \end{figure*}
Documents usually have a hierarchical structure formed by specific patterns, such as characters forming words which in-turn form sentences and paragraphs; similarly, cells and rows forming tables and combinations of sentences and tables creating forms etc. Since these patterns are often repeated in different parts of documents, there is a possibility of learning the structure of different types of documents as a collection of different local and global features. Various approaches for classification based on document structure have been proposed in the past. Most of these approaches consider specially designed local and global features along with their combinations for classification. These features suit specific types of documents and their performance is greatly effected when the document corpora change. Some approaches focus learning and optimizing features for different types of documents. These systems also perform diversely as the documents under question change. The biggest problem with such approaches is that for different types of documents, the feature sets and/or learning mechanisms need optimization. This becomes increasingly difficult as the document corpora grow. The situation becomes further challenging when we consider unconstrained documents, such as handwritten documents where a writer can freely write text, annotations, or equations, and draw tables or figures, etc.
The presence of unconstrained documents, both in terms of content or structure, demands approaches which are not largely affected by different structural hierarchy, contents, and spatial relationship among the parts of a document~\cite{lekang-14-a}.

In this paper we adapt deep Convolutional Neural Networks (CNN) model to the domain of unconstrained document classification. While CNN already show good performance for document classification, the little availability of huge training datasets limits their performance~\cite{lekang-14-a}. 
%The network adapted in the current paper is pre-trained using a huge image database, i.e.,  ImageNet~\cite{cnn_alexnet_nips2014}, containing millions of images according to the WordNet hierarchy where each node of the hierarchy is attributed by over $500$ images per node thereby totaling to $3.2$ million images. The images used for the pre-tarining are a subset of the ImageNet consisting of $1000$ categories and $1.2$ million images.
We initialize our network (except last fully connected layer) using weights from AlexNet which is trained on images from ImageNet~\cite{imagenet}.  ImageNet contains  millions of images according to the WordNet hierarchy where each node of the hierarchy is attributed by over $500$ images per node thereby totaling to $3.2$ million images. The AlexNet is trained on a subset consisting of $1000$ categories and $1.2$ million images.
The ImageNet contains general real world images of categories like, car, scooter, tiger, monkey, ship, etc., as shown in Figure~\ref{fig:ImageNet}(a). Note that the ImageNet has only one category, i.e., the \emph{Web} category containing some webpages which is somewhat similar to the traditional documents. Figure~\ref{fig:ImageNet}(b) shows the overall difficulty of the task by depicting some sample images from the Tobacco-3482 Legislation dataset on whom the proposed approach is evaluated.
Further, Figure~\ref{fig:TobaccoDoc} highlights the intra-class variations and inter-class similarities among three document classes: Ads, Forms, and Scientific writings, from the said dataset. However in this paper, similar to the state-of-the-art~\cite{lekang-14-a}, we classified the entire data in ten document classes:~\textit{news, letter, ad, note, scientific, form, email, memo, resume, and report}

It is important to mention the key differences between our approach and other CNN based approaches~\cite{lekang-14-a}. These are:
\begin{itemize}
\item For initialization, the proposed CNN model uses pre-trained weights from a network (AlexNet~\cite{cnn_alexnet_nips2014}) trained on $1.2$ million images from ImageNet.
\item The proposed network hierarchy is deeper than the network presented in~\cite{lekang-14-a}. Our approach contains $5$ convolutional layers in comparison to the $2$ convolutional layer model reported in~\cite{lekang-14-a}. This provides a lot more features ($4096$ instead of $1000$) to the fully connected layer for classification.
  \item AlexNet is trained on RGB images and extracts different types of features from each channel. We use the grey level image as input to all $3$ channels. It results in different types of feature extraction from same image for enriched feature hierarchies.
\end{itemize}

Our method outperforms the state-of-the-art method of document image classification (Le-Kang et al.~\cite{lekang-14-a}, $65.35\%$) and achieves the accuracy of $77.6\%$.
The superior results obtained by the presented approach signify the fact that visual recognition task share common visual cues. Note that the pre-training in the proposed approach does not involve document images used traditionally for document image classification.

\begin{figure*}
        \centering
        %\begin{subfigure}[b]{0.4\textwidth}
                \includegraphics[width=\textwidth]{deepdoc.pdf}
        %        \caption{}
        %        \label{fig:sample1}
        %\end{subfigure}%

        \caption{The Architecture of the deep convolutional neural network. The network is divided in conceptual blocks of convolutional and maxpooling layers for visualization. The only exception is the 3rd block which consists of $2$ convolutional layers.}
\label{fig:deepcnn}
\end{figure*}



